OverHear: Headphone based Multi-sensor Keystroke Inference

Headphones, traditionally limited to audio playback, have evolved to integrate sensors like high-definition microphones and accelerometers. While these advancements enhance user experience, they also introduce potential eavesdropping vulnerabilities, with keystroke inference being our concern in this work. To validate this threat, we developed OverHear, a keystroke inference framework that leverages both acoustic and accelerometer data from headphones. The accelerometer data, while not sufficiently detailed for individual keystroke identification, aids in clustering key presses by hand position. Concurrently, the acoustic data undergoes analysis to extract Mel Frequency Cepstral Coefficients (MFCC), aiding in distinguishing between different keystrokes. These features feed into machine learning models for keystroke prediction, with results further refined via dictionary-based word prediction methods. In our experimental setup, we tested various keyboard types under different environmental conditions. We were able to achieve top-5 key prediction accuracy of around 80% for mechanical keyboards and around 60% for membrane keyboards with top-100 word prediction accuracies over 70% for all keyboard types. The results highlight the effectiveness and limitations of our approach in the context of real-world scenarios.

==> mitigations.tex <==
\section{Mitigations}
\label{sec:mitigations}
The accuracy of inference attacks involving both microphones and accelerometers is closely linked to the sampling rate\cite{narain2014single}. \raveen{revisit}
To mitigate this risk, we can adjust the sampling rate specifically when the user is typing. This approach helps conserve resources and protect user privacy when the headset-connected application is active, while also maintaining regular sensor functionality and data quality when the headset is disconnected or the user is not engaged in typing. \raveen{revisit}

Furthermore, the utilization of noise-canceling headphones shows promise in diminishing background noises, including the audible clicks of keyboard presses noise-cancelling technology can be enhanced to not only reduce background noise but also identify and efficiently eliminate the distinct sound patterns produced by keyboard keystrokes. Although they may not entirely eliminate keyboard sounds, their use can result in a noticeable reduction in the accuracy of keystroke inference. 
Additionally, employing quieter keyboards, such as Scissor keyboards, can further mitigate such attacks. Scissor keyboards\cite{ScissorSwitchKeyboards}, often in laptops, offer a slim profile and quiet typing due to their scissor-like hinge structure. They outperform mechanical keyboards with audible switches and membrane keyboards with rubber domes by minimizing key-press noise. 
